John praised Mary because he? Implicit Causality Bias and Its Interaction with Explicit Cues in LMs

Some interpersonal verbs can implicitly attribute causality to either their subject or their object and are therefore said to carry an implicit causality (IC) bias. Through this bias, causal links can be inferred from a narrative, aiding language comprehension. We investigate whether pre-trained language models (PLMs) encode IC bias and use it at inference time. We find that to be the case, albeit to different degrees, for three distinct PLM architectures. However, causes do not always need to be implicit -- when a cause is explicitly stated in a subordinate clause, an incongruent IC bias associated with the verb in the main clause leads to a delay in human processing. We hypothesize that the temporary challenge humans face in integrating the two contradicting signals, one from the lexical semantics of the verb, one from the sentence-level semantics, would be reflected in higher error rates for models on tasks dependent on causal links. The results of our study lend support to this hypothesis, suggesting that PLMs tend to prioritize lexical patterns over higher-order signals.

==> sections/bertVgpt2.tex <==
\paragraph{find my place later}
The contrast between \gpttwo and \bert is quite enlightening as to the interaction between IC and EC. On average across congruent and incongruent stimuli, these two models perform comparably: 70.0\% accuracy for \bert and 71.2\% for \gpttwo. But as seen in Figure~\ref{fig:exp2}, under the hood they are behaving quite differently. In Figure~\ref{fig:np1-ratios} we saw another similarity between these two models: in the absence of an explicit cause, they both show an almost categorical preference for the object of the main clause. For \bert, the strength of this preference is modulated by IC considerably more than is the case for \gpttwo ($\rho=0.64$ v. $\rho=0.4$, resp.), but it is nevertheless favoring the object. In this experiment, we see the effect of the difference in IC bias awareness between the two models more clearly, specifically in how IC combines with EC to modulate the preference for the object. 

Table~\ref{tab:bertgpt2} shows a breakdown of the models' accuracy by IC and EC in their congruent and incongruent combinations. We see that both models are remarkably good at resolving the antecedent in the context of an object-related EC---this is not surprising considering the models' strong preference for the object in general. We do see, however, that \bert's preference for the object is lower in this context (S-O), compared to O-O, due to interference from the implicit S-bias of the verbs. In a similar pattern in the S-S condition, \bert seems to receive a boost in performance as both IC and EC signal to the model that it should overcome its strong preference for the object; while \gpttwo is left behind, presumably because the EC signal alone is not able to offset the preference for the object to the same degree. The O-S condition also corroborates this interpretation, this time with evidence of interference from the IC signal for \bert, which results in a lower performance for this model comapred to \gpttwo, which being less aware of IC bias is also less exposed to interference from it. 

For lack of space, we do not show this breakdown for the rest of the models, but we note that \electrasmall and \roberta pattern closely with \bert, only with a smaller gap between the pairs of congruent and incongruent conditions, due to a less extreme preference for the object in these models. While \electra and \electralarge show virtually no gaps of this kind, i.e. their preference for the object of the main clause, as seen in Figure~\ref{fig:np1-ratios}, being weaker in general, is completely overruled by IC and EC signals. 

\begin{table}[]
    \centering
    \resizebox{.48\textwidth}{!}{

    \begin{tabular}{l|lll|lll|l}
    \toprule
        & \multicolumn{3}{c}{Congruent} & \multicolumn{3}{c}{Incongruent} & All   \\
        \midrule
        & S-S & O-O & Ave & S-O & O-S & Ave & Ave\\
        \midrule
        \bert & 68.1 & 100.0 & 86.7 & 87.7 & 28.9 & 53.4 & 70.0 \\
        \gpttwo & 38.2 & 99.8 & 74.0 &96.7 & 48.1 & 68.4 & 71.2 \\
    \bottomrule
    \end{tabular}
    }
    \caption{IC-EC. EC is the correct bias. IC is the one that either enhances or interferes with EC.}
    \label{tab:bertgpt2}
\end{table}

==> sections/plots_galore.tex <==
\begin{figure}[htbp!]
    \centering
    \includegraphics[width=0.95\linewidth]{acl2020-templates/sections/images/experiment-1.pdf}
    \caption{Experiment 1 result.}
    \label{fig:exp1}
\end{figure}

\begin{figure}[htbp!]
    \centering
    \includegraphics[width=0.95\linewidth]{acl2020-templates/sections/images-wugs/experiment-1-wugs.pdf}
    \caption{Experiment 1 result with wug data.}
    \label{fig:exp1-wugs}
\end{figure}





\begin{figure*}[htbp!]
    \centering
    \includegraphics[width=0.95\linewidth]{acl2020-templates/sections/images/correlations-models.pdf}
    \caption{Model to human agreement.}
    \label{fig:correlations}
\end{figure*}




\begin{figure*}[htbp!]
    \centering
    \includegraphics[width=0.95\linewidth]{acl2020-templates/sections/images/categories-models.pdf}
    \caption{Semantic categories.}
    \label{fig:categories}
\end{figure*}

\begin{figure*}[htbp!]
    \centering
    \includegraphics[width=0.95\linewidth]{acl2020-templates/sections/images-wugs/categories-models-wugs.pdf}
    \caption{Semantic categories with wug data.}
    \label{fig:categories-wugs}
\end{figure*}



\begin{figure*}[htbp!]
    \centering
    \includegraphics[width=0.95\linewidth]{acl2020-templates/sections/images/valency-models.pdf}
    \caption{Valency rating.}
    \label{fig:valency}
\end{figure*}

\begin{figure*}[htbp!]
    \centering
    \includegraphics[width=0.95\linewidth]{acl2020-templates/sections/images-wugs/valency-models-wugs.pdf}
    \caption{Valency rating with wug data.}
    \label{fig:valency-wugs}
\end{figure*}

\begin{figure*}[htbp!]
    \centering
    \includegraphics[width=0.95\linewidth]{acl2020-templates/sections/images/congruency.pdf}
    \caption{Congruent and incongruent antecedent resolution.}
    \label{fig:congruency}
\end{figure*}

\begin{table}[hbtp!]
    \centering
    \small
    \begin{tabular}{l|rrrr}
    
   &  \multicolumn{1}{c}{he}   & \multicolumn{1}{c}{she} &  \multicolumn{1}{c}{he w/ verb}   & \multicolumn{1}{c}{she w/ verb} \\
   \hline
    bookcorpus & 87,492 & 61,002 & 9,781 & 6,900\\
    wikipedia  & 66,429 & 25,493 & 54,727 & 20,936\\
    \end{tabular}
    \caption{"because he" and "because she" counts}
    \label{tab:because_pron}
\end{table}

==> sections/todos.tex <==
- cite shit
- discuss absolute ranking of he/she in Exp1 and 3
- write section on choice of referent
- change title
- run exps with electra tiny - with final checkpoint first - if evidence of bias, with intermediate ones too
- establish baselines
- shows Exp 2 results in a plot
- do we want to disucss gender effects? if not, get rid of all gender results in tables
- discuss corpus study findings
- think/talk about the word bias
- fig 2: change NP1 - NP2 to S-O
- decide whether to keep 26/50s or not
